Kernelized Hashcode Representations for Relation Extraction

Kernel methods have produced state-of-the-art results for a number of NLP tasks such as relation extraction, but suffer from poor scalability due to the high cost of computing kernel similarities between natural language structures. A recently proposed technique, kernelized locality-sensitive hashing (KLSH), can significantly reduce the computational cost, but is only applicable to classifiers operating on kNN graphs. Here we propose to use random subspaces of KLSH codes for efficiently constructing an explicit representation of NLP structures suitable for general classification methods. Further, we propose an approach for optimizing the KLSH model for classification problems by maximizing an approximation of mutual information between the KLSH codes (feature vectors) and the class labels. We evaluate the proposed approach on biomedical relation extraction datasets, and observe significant and robust improvements in accuracy w.r.t. state-of-the-art classifiers, along with drastic (orders-of-magnitude) speedup compared to conventional kernel methods.

==> algo_opt_hash_config.tex <==
% 
\begin{algorithm}[tp!]
\caption{
% \csize
\csizenine
% 
KLSHOptimizeConfigurationSupervised
% 
% Optimizing Configuration Parameters of a Kernel-Hashing Model along with an Ensemble Classifier
% 
}
% \scriptsize
\csizenine
% \csize
% \small
\begin{algorithmic}[1]
\REQUIRE Training dataset, $\{ \bs{S}, \bs{y} \}$; Reference set of constant size $M \ll N$, $\bs{S}^R$; number of samples from set $\bs{S}$ for computing MI LB, $\gamma$; kernel similarity function, $K(., .)$.
% 
\STATE $\bs{K}_{R} \gets$ computeKernel($\bs{S}$, $\bs{S}^R$, $K(.,.)$)
\label{algline:kernel_compute}
\COMMENT{$N\!\times\!M$ size}
% \COMMENT{kernel similarities for $O(N)$ pairs of NLP structures}
% \\
% 
% \STATE \COMMENT{choice of a hashing function, $f_{\mhk}$}
% \FOR{$f_{\mhk} \in$ \{ Kulis, RkNN, RMM \}}
% \label{algline:opt_hash}
%
% 
% \STATE 
% \COMMENT{Choices for $\alpha$ can be s.t. $\alpha < M^{\frac{1}{2}}$}
% 
% \FOR{$\alpha \in$ \{ 1, 2, 3, 4, 5, 8, 10, 15, 20 \}}
% 
% \FOR{$H \in$ \{ 100, 300, 1000\}}
% 
\FOR{$f_{\mhk} \in$ \{ Kulis, RkNN, RMM \}, $\alpha \in$ \{ 1, 2, $\cdots$, $M^{\frac{1}{2}}$\}, $H \in$ \{100, $\cdots$, 1000\}}
\label{algline:opt_hash}
% 
\STATE $\bs{r}^{lb}$ $\gets$ randomSubset($N$, $\gamma$)
\label{algline:sample_config_milb}
\COMMENT{$\gamma$ samples from $\{N\}$}
% 
\STATE $\bs{C} \gets$ kernelHashing($\bs{K}_R(\bs{r}^{lb})$, $f_{\mhk}, \alpha, H$)
\label{algline:klsh_config_compute}
% \COMMENT{$O(H)$}
% 
% \FOR{$j=1 \to H$}
% \STATE $\bs{r}^{h}_{j} \gets$ randomSubset($M$, $2\alpha$)\\
% \ENDFOR
% 
\STATE 
\COMMENT{$\eta$=None refers to bagging based ensemble}
\FOR{$R \in$ \{ 1, $\cdots$, 250 \}, $\eta \in$ \{ None, 5, $\cdots$, 30 \}}
% 
% 
% ~(subset of data) 
% is trained 
% instead of taking subset of hashcode bits
% \FOR{$\eta \in$ \{ None, 5, 10, 15, 20, 30 \}}
% 
\STATE $mi_{lb} \gets$ computeMILB($\bs{C}, \bs{y}(\bs{r}^{lb}), R, \eta$)
\label{algline:milb_config}
% 
\STATE Store $\{f_{\mhk}, \alpha, H, R, \eta\}$ and $mi_{lb}$
% 
% \STATE Store configuration if higher MI LB.
% 
% \ENDFOR
% 
% \ENDFOR
% 
% \ENDFOR
% 
\ENDFOR
% 
\ENDFOR
% 
% \STATE \COMMENT{$f_{\mhk}^*, \alpha^*, H^*$ are optimized parameters for hashing}
\STATE $\bs{C} \gets$ kernelHashing($\bs{K}_R, f_{\mhk}^*, \alpha^*, H^*$)\COMMENT{recompute hashcodes with optimized configuration~(maximum MI LB)}
% 
\RETURN optimized configuration and hashcodes $\bs{C}$
% of $\bs{S}$ for the configuration.
\label{algline:return_opt_hash}
% 
\end{algorithmic}
\label{alg:opt_hash_config}
\end{algorithm}
% 


==> hash_algo.tex <==
\begin{algorithm}[th]
\caption{
\small
 Algorithm for Computing KLSH Codes.}
\small
\begin{algorithmic}[1]
\REQUIRE Kernel similarity vector $\bs{k}$ of size $M$, computed for a structure $S$; sub-sampling parameter, $\alpha$, for randomizing hash function; the number of hash functions, $H$.
\COMMENT{Random subsets, fixed across structure inputs}
\FOR{$j=1 \to H$}
\STATE $\bs{r}^{h}_{j_1} \gets$ randomSubset($M$, $\alpha$)
\STATE $\bs{r}^{h}_{j_2} \gets$ randomSubset($M$, $\alpha$)
\ENDFOR
\STATE $\bs{c} \gets \bs{0}$
\FOR{$j=1 \to H$}
\STATE $\bs{k}_{j_1} \gets \bs{k}(\bs{r}^{h}_{j_1})$
\STATE $\bs{k}_{j_2} \gets \bs{k}(\bs{r}^{h}_{j_2})$
\IF{min($\bs{k}_{j_1}$) $<$ min($\bs{k}_{j_2}$)}
\STATE $\bs{c}(j) \gets 0$
\ELSE
\STATE $\bs{c}(j) \gets 1$
\ENDIF
\ENDFOR
\RETURN $\bs{c}$
\end{algorithmic}
\label{alg:our_algo_klsh_codes}
\end{algorithm}


==> klsh_hash_algo.tex <==
% \begin{algorithm}[tp!]
% \caption{
% \csizenine
% % 
% GeneralizedKLSH
% % 
% % Generalized Pseudo Code for Building Locality Sensitive Hash Functions using Kernel Similarities
% % 
% % Compute Random-kNN KLSH Code~[Garg et al., 2018]
% }
% % 
% \csizenine
% % 
% \begin{algorithmic}[1]
% \REQUIRE Reference set of NLP structures, $\bs{S}^R
% \in \{ S_1, \cdots, S_M \}$;
% sub-sampling parameter, $\alpha$; number of hash functions, $H$; kernel similarity function, $K(., .)$.
% % , computing similarity between two language structures.
% \STATE $\bs{K}_{RR} \gets$ computeKernel($\bs{S}^R$, $\bs{S}^R$, $K(.,.)$)\COMMENT{$M \times M$}
% % 
% \FOR{$j=1 \to H$}
% \STATE $\bs{r}^{h}_{j} \gets$ randomSubset($M$, $2\alpha$)\COMMENT{sample $2\alpha$ elements randomly from set $\{1, \cdots, M\}$}
% % 
% \STATE $h_j(.) \gets$ buildKernelHashFunction($\bs{K_{RR}},\bs{r}^{h}_{j}$, $f_{\mhk}$)
% \label{algline:hashfunc}
% \COMMENT{kernel-hashing choices: RkNN, RMM, Kulis}
% % 
% \ENDFOR
% \RETURN $h_1(.), \cdots, h_H(.)$
% \end{algorithmic}
% \label{alg:general_algo_klsh_codes}
% \end{algorithm}
% 
% 
% 
% 
% 
% 
\begin{algorithm}[tp!]
\caption{
\csizenine
% 
KLSH
% 
% Generalized Pseudo Code for Building Locality Sensitive Hash Functions using Kernel Similarities
% 
% Compute Random-kNN KLSH Code~[Garg et al., 2018]
}
% 
\csizenine
% 
\begin{algorithmic}[1]
\REQUIRE An input set of data points $\bs{S}$ of size $N$, the reference set $\bs{S}^R$, and the kernel function parameters $\bs{\theta}$.
% , computing similarity between two language structures.
\STATE $\bs{K} \gets K(\bs{S}, \bs{S}^R; \bs{\theta}))$
\COMMENT{$N \times M$ kernel computations}
\FOR{$i=1 \to N$}
\STATE $\bs{c}_i \gets \bs{h}(\bs{k}_i)$
\ENDFOR
\RETURN \bs{C}
\end{algorithmic}
\label{alg:algo_klsh_code}
\end{algorithm}
% 
% 

==> klsh_kulis.tex <==
\begin{algorithm}[tp!]
\caption{
\csizeten
Kernelized Locality Sensitive Hash Function~\cite{kulis2009kernelized}
}
% 
\csizeten
% 
\begin{algorithmic}[1]
\REQUIRE Reference set of natural language structures, $\bs{S}^R
\in \{ S_1, \cdots, S_M \}$;
sub-sampling parameter, $\alpha$; number of hash functions, $H$; convolution-kernel function, $K(., .)$, computing similarity between two language structures.
% vector $\bs{k}$ of size $M$, computed for a structure $S$; 
% 
% sub-sampling parameter, $\alpha$, for randomizing each of the $H$ hash functions.
% 
% ; the number of hash functions, $H$.
% \FOR{$j=1 \to H$}
% \STATE $\bs{r}^{h}_{j_1} \gets$ randomSubset($M$, $\alpha$);\ \ $\bs{r}^{h}_{j_2} \gets$ randomSubset($M$, $\alpha$)
% % \STATE $\bs{r}^{h}_{j_2} \gets$ randomSubset($M$, $\alpha$)
% \ENDFOR
\STATE $\bs{K}_{RR} \gets$ computeKernel($\bs{S}^R$, $\bs{S}^R$)
\COMMENT{$M \times M$}\\
% 
% ;\ \ \ 
% \STATE $\bs{c} \gets \bs{0}_{H}$
% \STATE $\bs{c} \gets \bs{0}_{H}$
% 
\FOR{$j=1 \to H$}
\STATE $\bs{r}^{h}_{j} \gets$ randomSubset($M$, $2\alpha$)\\
% 
% \COMMENT{random subsets, fixed across structure inputs}
% 
% \STATE $\bs{k}_{j_1} \gets \bs{k}(\bs{r}^{h}_{j_1})$;\ \ $\bs{k}_{j_2} \gets \bs{k}(\bs{r}^{h}_{j_2})$
% 
% \STATE $\bs{k}_{j_2} \gets \bs{k}(\bs{r}^{h}_{j_2})$
% 
\STATE $\cH_j \gets$ buildKernelHashFunction($\bs{K_{RR}}(\bs{r}^{h}_{j}, \bs{r}^{h}_{j})$)
% 
% \STATE \textbf{if} max($\bs{k}_i(\bs{r}^{h}_{j_1})$) $>$ max($\bs{k}_i(\bs{r}^{h}_{j_2})$) 
% \textbf{then} 
% \\
% \ \ \ \ 
% $\bs{c}(j) \!\gets\! 0$ 
% \\
% \textbf{else} 
% \\
% \ \ \ \ 
% $\bs{c}(j) \!\gets\! 1$ 
% \\\textbf{endif}
% 
% \STATE \textbf{if} min($\bs{k}_{j_1}$) $<$ min($\bs{k}_{j_2}$) \textbf{then} $\bs{c}(j) \gets 0$ \textbf{else} $\bs{c}(j) \gets 1$ \textbf{end if}
% 
% \IF{min($\bs{k}_{j_1}$) $<$ min($\bs{k}_{j_2}$)}
% \STATE $\bs{c}(j) \gets 0$
% \ELSE
% \STATE $\bs{c}(j) \gets 1$
% \ENDIF
% 
\ENDFOR
% \RETURN $\bs{c}$
\RETURN $\cH_1, \cdots, \cH_H$
\end{algorithmic}
\label{alg:our_algo_klsh_codes}
\end{algorithm}
% 
% 

==> math_commands.tex <==
\newcommand{\cA}{{\mathcal{A}}}
\newcommand{\cB}{{\mathcal{B}}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\cG}{{\mathcal{G}}}
\newcommand{\cI}{{\mathcal{I}}}
\newcommand{\cN}{{\mathcal{N}}}
\newcommand{\cM}{{\mathcal{M}}}
\newcommand{\cO}{{\mathcal{O}}}
\newcommand{\cP}{{\mathcal{P}}}
\newcommand{\bP}{{\mathbf{P}}}
\newcommand{\cR}{{\mathcal{R}}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cH}{{\mathcal{H}}}
\newcommand{\cK}{{\mathcal{K}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\cU}{{\mathcal{U}}}
\newcommand{\cV}{{\mathcal{V}}}
\newcommand{\cY}{{\mathcal{Y}}}
\newcommand{\newsetminus}{{\!-\!}}
\newcommand{\cVmA}{{\cV\newsetminus\cA}}
\newcommand{\cX}{{\mathcal{X}}}
\newcommand{\cs}{s}
\newcommand{\cVms}{{\cV-\cs}}

\newcommand{\ba}{{\mathbf{a}}}
\newcommand{\bb}{{\mathbf{b}}}
\newcommand{\bu}{{\mathbf{u}}}
\newcommand{\bx}{{\mathbf{x}}}
\newcommand{\resid}{\cR}

\newcommand{\NP}{{\mathbf{NP}}}

% \DeclareMathOperator{\MIF}{MI} 

\newcommand{\bs}[1]{\boldsymbol{#1}}

\newcommand{\mhk}{\cM^h_k}

\newcommand{\thmref}[1]{Theorem~\ref{#1}}
\newcommand{\tabref}[1]{Tab.~\ref{#1}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\eqnref}[1]{(Eq. \ref{#1})}
\newcommand{\secref}[1]{Sec.~\ref{#1}}
\newcommand{\appref}[1]{Appendix~\ref{#1}}
\newcommand{\prcref}[1]{Procedure~\ref{#1}}
\newcommand{\assmref}[1]{Assumption~\ref{#1}}
\newcommand{\crlref}[1]{Corollary~\ref{#1}}
\newcommand{\algoref}[1]{Alg.~\ref{#1}}
\newcommand{\prpref}[1]{Proposition~\ref{#1}}
\newcommand{\cnjref}[1]{Conjecture~\ref{#1}}
\newcommand{\axmref}[1]{Axiom~\ref{#1}}
\newcommand{\lmaref}[1]{Lemma~\ref{#1}}

\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}[lemma]{Corollary}
\newtheorem{procedure}[lemma]{Procedure}
\newtheorem{assumption}[lemma]{Assumption}
\newtheorem{claim}[lemma]{Claim}
\newtheorem{conclusion}[lemma]{Conclusion}
\newtheorem{proposition}[lemma]{Proposition}
\newtheorem{conjecture}[lemma]{Conjecture}
\newtheorem{axiom}[lemma]{Axiom}
\newtheorem{algo}[lemma]{Algorithm}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}


\newcommand{\mai}{ODL }
\newcommand{\nmai}{NODL+ }
\newcommand{\gmai}{NODL- }
\newcommand{\ngmai}{NODL }
%
\newcommand{\mains}{ODL}
\newcommand{\nmains}{NODL+}
\newcommand{\gmains}{NODL-}
\newcommand{\ngmains}{NODL}

%additions suggested by Sahil
\newcommand{\s}[1]{\textcolor{magenta}{#1}}
%deletions suggested by Sahil
\newcommand{\sd}[1]{\textcolor{orange}{#1}}


==> nonstationary_par.tex <==
% \paragraph{Nonstationary Convolution Kernel Parameters}
% 
% \label{sec:nonstationary_kernel}
% 
% 
% We propose a generic approach to extend any convolution kernel to a non-stationary one, for higher expressibility and generalization.
% % 
% \begin{definition}[Stationary kernel~\cite{genton2001classes}]
% A \emph{stationary} kernel, between vectors $\bs{x}_i, \bs{x}_j \in \mathbb{R}^d$, is the one which is translation invariant:
% % 
% % \vspace{-1.5mm}
% \begin{align*}
% k(\bs{x}_i, \bs{x}_j) = k^S(\bs{x}_i - \bs{x}_j),
% % \vspace{-3mm}
% \end{align*}
% \noindent that means, it depends only upon the lag vector between $\bs{x}_i$ and $\bs{x}_j$, and not the data points themselves.
% % \vspace{-5.5mm}
% \label{def:stationary_kernel}
% \end{definition}
% % 
% For NLP context, 
% stationarity in convolution kernels is formalized in \thmref{thm:st_conv}.
% % 
% 
% \begin{theorem}
% A convolution kernel $K(.,.)$, a function of the kernel $k(.,.)$, is stationary if $k(.,.)$ is stationary.
% % \vspace{-2mm}
% % 
% % \begin{proof}[Proof Sketch]	 
% % Suppose we have a vocabulary set, $\{ l_1, \cdots, l_{p}, \cdots, l_{2p} \}$, and we randomly generate a set of discrete structures $\mathcal{X} = \{ X_1, \cdots,  X_N \}$, using $l_1, \cdots, l_p$. For kernel $k(.,.)$, that defines similarity between a pair of labels, consider a case of stationarity, $k(l_i,l_j) = k(l_{i+p}, l_{j}) = k(l_{i}, l_{j+p}); i,j \in \{1, \cdots, p\}$, where its value is invariant w.r.t. to the translation of a label $l_i$ to $l_{i+p}$. 
% % In the structures, replacing labels $l_1, \cdots, l_p$ with $l_{p+1}, \cdots, l_{2p}$ respectively, we obtain a set of new structures $\bar{\mathcal{X}} = \{ \bar{X}_1, \cdots, \bar{X}_N \}$. Using a convolution kernel $K(.,.)$, as a function of $k(.,.)$, we obtain same~(kernel) Gram matrix on the set $\bar{\mathcal{S}}$ as for $\mathcal{S}$. Thus $K(.,.)$ is also invariant w.r.t. the translation of structures set $\mathcal{S}$ to $\mathcal{\bar{S}}$, hence a stationary kernel~(Def. \ref{def:stationary_kernel}).
% % \end{proof}
% % 
% \label{thm:st_conv}
% % \vspace{-3mm}
% \end{theorem}
% 	
% % \todo{The work emphasizes that the new kernel is nonstationary; however, this fact
% % is not used in the paper. Yes, it is important to establish that the
% % extension is a valid kernel, but nonstationary property, in fact, depends on
% % the properties of the underling extended kernel. For example, if k(i, j) is
% % the indicator function in Theorem 2, then the proof is not valid.}

% Some examples of kernels $k(.,.)$ are:
% % \vspace{-2.5mm}
% \begin{align*}
% &
% k(i, j) = \mathbb{I}(i = j),\ 
% k(i,j) = \exp(-||\bs{w}_i - \bs{w}_j||_2^2),
% \\
% &
% k(i,j) = \exp(\bs{w}_i^T\bs{w}_j-1).
% % \vspace{-7.5mm}
% \end{align*}
% % 	
% \noindent Herein, $i, j$ are words~(node/edge labels), and $\bs{w}_i$, $\bs{w}_j$ are word vectors respectively; $\mathbb{I}(.)$ is an indicator function. The first two kernels are stationary. Whereas the third one is non-stationary, mathematically, though it relies only on the cosine similarity between the word vectors, not the word-vectors or words themselves.
% % 
% Our approach is generic enough for not only extending a stationary convolution kernel, but a non-stationary convolution kernel as well, accounting for the cases as the latter one, for a higher flexibility and generalization.
% %  
% % 
% \begin{theorem}
% Any convolution kernel $K(.,.)$, can be extended to a valid non-stationary convolution kernel $K^{NS}(.,.)$, by extending the kernel function $k(.,.)$ to $k^{NS}(.,.)$ as in \eqnref{eqn:ns_ext}, with a deterministic function $\sigma(.)$ of any form.
% %
% % \vspace{-1.5mm}
% \begin{align}
% k^{NS}(i,j) = \sigma(i) k(i,j) \sigma(j)
% % \vspace{-5.5mm}
% \label{eqn:ns_ext}
% \end{align}
% % \begin{proof}[Proof Sketch]
% % % 
% % The extended kernel function $k^{NS}(i,j)$ is a valid kernel~\cite[p. 95]{rasmussen2006gaussian}, and therefore, $K^{NS}(.,.)$, as a function of $k^{NS}(.,.)$, is also a valid convolution kernel. For establishing the nonstationarity property, following the proof of \thmref{thm:st_conv}, if using $K^{NS}(.,.)$,
% % % ,
% % we obtain a (kernel) Gram matrix on the set $\bar{\mathcal{S}}$ that is different from the set $\mathcal{S}$ because $\sigma(l_i) \neq \sigma(l_{i+p}) \ \forall i \in \{ 1, \cdots, p \}$ for an arbitrary selection of $\sigma(.)$. Therefore $K^{NS}(.,.)$ is not invariant w.r.t. the translation of set $\mathcal{S}$ to $\mathcal{\bar{S}}$, hence a nonstationary kernel~(Def. \ref{def:stationary_kernel}). 
% % \end{proof}
% % \vspace{-2mm}
% \end{theorem}
% 	
% In natural language modeling problems, since $k(.,.)$ operates on labels~(or a tuple of labels), $\sigma(.)$ can be thought of as 1-D embedding of the vocabulary for labels. For $\sigma(.) \in \mathbb{R}_{\geq 0}$, it is like the strength of a label in the context of computing the convolution kernel similarity. \emph{For instance, if $\sigma(i)=0$, it means that the label $i$ should be completely ignored when computing a convolution kernel similarity of a discrete structure~(tree, path, etc.), that contains the (node or edge) label $i$, w.r.t. another discrete structure, or itself.}
% %	
% Thus, we see that these additional parameters, introduced with the nonstationary model, allow convolution kernels to be expressive enough to decide if some substructures in a discrete structure should be ignored. One can also define $\sigma(.)$ on the vector space representation of the labels~(word vectors), like $\sigma(\bs{w}_i)$ instead of $\sigma(i)$. 
% 
% 
% \paragraph{Nonstationarity for Skipping Sub-structures}
% Suppose we are interested in computing the convolution kernel similarity between the paths of tuples ---as in \tabref{tab:semantic_attention} or between the two trees in \tabref{fig:amr_valid_extraction}, \ref{fig:amr_invalid_extraction}. In both cases, the basic kernel function, $k(.,.)$ operates on a pair of tuples. 
% 	
For path kernels, or graph kernels, the nonstationary kernel on tuples can be defined as:
%
% \vspace{-1mm}
\begin{align*}
% $
% &
% \tabsize
k^{NS}
\!
((e_i, n_i),\! (e_j, n_j))
% \!
= 
% \!
% \sigma_(e_i)
\sigma_{e_i}
k_e(e_i, e_j)
% \sigma(e_j)
\sigma_{e_j}
k_n(n_i, n_j).
% $
% 
% \vspace{-2mm}
\end{align*}
% %
% In the above expression, 
\noindent 
The similarity between two tuples $(e_i, n_i)$ and $(e_j, n_j)$ is defined as the product of kernels on the edge labels $e_i, e_j$ and the node labels $n_i, n_j$.
% % The kernel functions $k_e(e_i, e_j)$ and $k_n(n_i, n_j)$ can be thought of as black boxes in our approach; however, 
% In our experiments, we consider the following functions: 
% % 
% % \vspace{-3mm}
% \begin{align*}
% &
% \csize
% k_e(e_i, e_j) = \mathbb{I}(e_i = e_j),\ \  
% k_n(n_i, n_j) = \mathbb{I}(n_i = n_j),\\
% &
% \csize
% k_n(n_i, n_j) \!=\! \exp(\bs{w}_{n_i}^T\bs{w}_{n_j}\!-\!1)((\bs{w}_{n_i}^T\bs{w}_{n_j} \!-\! \gamma)/(1\!-\!\gamma))_{+}.
% % \vspace{-5mm}
% \end{align*}
% \noindent Herein, $(.)_{+}$ denotes the positive part; $\gamma \in (-1, 1)$ is a sparsity parameter.
 
% We consider the nonstationary parameters to be binary valued, i.e., $\sigma \in \{ 0, 1 \}$~(we keep binary values only, as a measure for robustness to over-fitting, as well as for keeping the optimization simple).
% % 
	
% In the expression above, non-stationarity parameters are local to edge labels~(referred as semantic labels in this paper), which come from a language representation~(predefined, and small in vocabulary), such as Abstract Meaning Representations~\cite{banarescu2012abstract}, Stanford Dependencies~\cite{chen2014fast}, etc. 
% % 
% Defining the $\sigma$ parameters local w.r.t. the edge labels~(semantic labels), corresponds to attention on the semantics in the context of convolution kernel computation. 
% % 	
% For instance, as shown in \tabref{tab:semantic_attention}, 
% we find that it is more optimal to skip tuples, containing either of the semantic labels \emph{arg2, arg0, op2, example} when computing convolution kernel similarity, as $\sigma=0$ for all these labels in our learned model for the task.~\footnote{arg0, arg2 are not ignored if duplicate data points are kept.
% % 	
% Thus, our proposed nonstationary approach allows decisions on what to attend in a linguistic representation of a natural language, and what not to attend. This is very intuitive, as it is close to how a human mind processes natural language.
	
% \todo{Try to simplify the notations.}
% 
% \todo{this is different from optimizing the hash functions individually as done in some of the works, which are not LSH.}
	

==> ppi_evaluation.tex <==
\begin{table}[tp!]
\centering
\csize
% 
\begin{tabular}{lll}
		\toprule
		\textbf{Models}
%        
&\textbf{(A, B)}&\textbf{(B, A)}\\
% 
        \toprule
% 
SVM$_1$~(Airola08)&0.25&0.44\\
% \midrule
% 
SVM$_2$~(Airola08)&0.47&0.47\\
\midrule
%
SVM~(Miwa09)&0.53&0.50\\
\midrule
% 
SVM~(Tikk10)&0.41&0.42\\
&(0.67, 0.29)&(0.27, 0.87)\\
% 
% \midrule
% PIPE~(Chang16)
% &\textbf{0.58}&\textbf{0.52}\\
% 
% \midrule
% % % % full features set
% kNN&$0.51$&$0.54$\\
% &(0.40, 0.72)&(0.39, 0.85)\\
% % 
% % \midrule
% % P-P shortest paths features set
% % kNN&$0.34$&$0.40$\\
% % &(0.47, 0.26)&(0.46, 0.36)\\
% 
\toprule
CNN~(Peng17)
&0.48&0.50\\
&(0.40, 0.61)&(0.40, 0.66)\\
\midrule
% 
RNN~(Hsieh17)
&0.49&0.51\\
% &(0., 0.)&(0., 0.)\\
% 
%
\midrule
CNN-RevGrad~(Ganin16-Rios18)
&0.43&0.47\\
%
\midrule
Bi-LSTM-RevGrad~(Ganin16-Rios18)
&0.40&0.46\\
% 
\midrule
Adv-CNN~(Rios18)
&0.54&0.49\\
% 
\midrule
Adv-Bi-LSTM~(Rios18)
&$\bs{0.57}$&0.49\\
% % 
% % full features set
\midrule
KLSH-kNN&$0.51$&$0.51$\\
&(0.41, 0.68)&(0.38, 0.80)\\
% 
% \midrule
% KLSH-kNN-NS*&$\bs{}$&$$\\
% 
% 
% 
% P-P shortest paths
% \midrule
% KLSH-kNN*&$0.$&$0.$\\
% % &(0., 0.)&(0., 0.)\\
% 
% \toprule
% % % 0.25
% % M=500, full features set, R=250, alpha=20
% \textbf{KLSH-RF*}&$\bs{0.54}$&$\bs{0.52}$\\
% &(0.39, 0.86)&(0.35, 0.97)\\
% %
% 
% infer prob. fixed to 0.25 for cross-corpus evaluation
% optimized hash config.
% M=500, full features set, R=250, alpha=5, H=100
% optimized hash config.
% M=500, full features set, R=250, alpha=3, H=100
%
% \midrule
% 
% \textbf{KLSH-RF*}&$\bs{0.56}$&$\bs{0.53}$\\
% &(0.45, 0.75)&(0.37, 0.93)\\
% % 
% 
% % 
% % 
% % infer prob. fixed to 0.25 for cross-corpus evaluation
% % optimized hash config.
% % todo: revise configs.
% % M=500, full features set, R=100, alpha=5, H=100
% % optimized hash config.
% % M=500, full features set, R=100, alpha=3, H=100
% % 
% % 
% \midrule
% \textbf{KLSH-RF}&$\bs{0.57}$&$\bs{0.53}$\\
% &(0.46, 0.74)&(0.37, 0.93)\\
% % 
% 
\toprule
% RMM
% p0.25
% M=500
% optimizing kernel, but fixed hash parameters
% AIMed -> BioInfer
% H=1000, R=250, alpha=2
% 
% p0.35
% BioInfer -> AIMed
% H=1000, R=250, alpha=2
\textbf{KLSH-RF}
% $^{+}$
&$\bs{0.57}$&$\bs{0.55}$\\
&(0.46, 0.75)&(0.45, 0.71)\\
% % 
% 
% 
% % fasttext
% % infer prob. fixed to 0.25 for cross-corpus evaluation
% % optimized hash config.
% % optimized RMM amongst three
% % M=500, full features set, R=100, alpha=3, H=1000, bagging
% % optimized hash config.
% % optimized to RkNN amongst three
% % M=500, full features set, R=250, alpha=1, H=1000, bagging
% %
% \midrule
% % 
% \textbf{KLSH-RF*}&$\bs{0.55}$&$\bs{0.54}$\\
% &(0.43, 0.73)&(0.37, 0.95)\\
% 
% 
% 
% (AIMed-BioInfer, tuned with validation 10% set) M=500, alpha=20, full features set, 0.25, R=250
% (BioInfer-AIMed, tuned with validation 10% set) M=500, alpha=20, full features set, 0.3, R=100
% \textbf{KLSH-RF*}&$\bs{0.54}$&$\bs{0.53}$\\
% &(\textbf{0.39, 0.86})&(\textbf{0.37, 0.94})\\
% 
% 
% 0.25
% M=500, P-P shortest paths features set, R=250, alpha=20
% \textbf{KLSH-RF*}&$\bs{0.53}$&$\bs{0.53}$\\
% &(\textbf{0.37, 0.91})&(\textbf{0.37, 0.91})\\
% 
% 
% % M=100, full features set, R=1000, alpha=20
% KLSH-RF*~(Ours)&$\bs{0.55}$&$\bs{0.52}$\\
% &(\textbf{0.41, 0.84})&(\textbf{0.35, 0.97})\\
\toprule
\end{tabular}
% \vspace{-3.5mm}
\caption{
Cross-corpus evaluation results for (training, test) pairs of PPI datasets, AIMed~(\textbf{A}) and BioInfer~(\textbf{B}) datasets. For each model, we report F1 score in the first row corresponding to it. In some of the previous works, precision, recall numbers are not reported; wherever available, we show precision, recall numbers as well, in brackets. Here, ``Ganin16-Rios18" means that the model is originally proposed in \protect\cite{ganin2016domain}, and evaluated for these datasets by \protect\cite{rios2018generalizing}.
}
\vspace{-3mm}
\label{tab:results_ppi}
\end{table}


==> problem_statement.tex <==
\vspace{-2.5mm}
\section{
% Problem Specification
Bio-Medical Relation Extraction Task
\& Problem Statement
}
\label{sec:ps}
\vspace{-1.75mm}
% 
% 
In this paper, we consider the problem of extracting information on bio-molecular interactions from text sentences. See \figref{fig:sdg_extraction} for an example of extractions.
%  
A single bio-molecular interaction has an interaction type~(possibly, from an unrestricted list of interaction types), and one or two entities participating in the interaction, and optionally one entity acting as a catalyst for the interaction
~\cite{airola2008all,hakala2013evex,garg2016extracting}.
% ~\cite{airola2008all,tikk2010comprehensive,hakala2013evex,garg2016extracting,raobiomedical,peng2017deep,hsieh2017identifying,garg2018stochastic}.

As per this specification of a bio-molecular interaction, from the lists of tokens identified as bio-entities and interaction types in a sentence, one can automatically enumerate over all candidate extractions.
% Some of those should be valid, and the rest, invalid. 
For each sentence in training set, an annotator manually annotates which of the candidate extractions are valid or invalid.
% 
% while a complete list of candidates is generated automatically.
% 
Thus, our problem is of binary classifying if a candidate extraction is valid or not, using the test sentence along with its syntactic/semantic parses as NLP features. 
% 	
Specifically, in reference to \figref{fig:klsh_rf}, from the syntactic~(semantic) parse of a sentence, a (post-processed) subgraph is obtained for each candidate extraction that is binary classified as a proxy for the candidate itself; one can obtain a path of tuples~(path-tuples) via traversal of a subgraph, for use with classification models which operate on sequences rather than graphs.
% 
% Basically, the problem is of classifying NLP structures for the bio-medical extraction task explained above.
% 	
% Basically, 
% For the purpose of understanding the generic algorithmic contributions of this paper, 
	
\input{tab_notations.tex}
% 
Conforming to the task specification, we consider a problem of classifying NLP structures, such as sequences, paths, graphs, etc. Let $\bs{S} = \{ S_i \}_{i=1}^N$ be a set of NLP structures, or data points, with their corresponding class labels, $\bs{y} = \{ y_i \}_{i=1}^N$. Our goal is we infer the class label of a given test data point $S_*$.
% 
% These bio-information extraction tasks become even more challenging when using a noisy list of bio-entities or interaction types rather than gold annotations, as in real world deployments.
	
% In some older datasets, task is somewhat simpler of just identifying pairs of interacting entities while ignoring the interaction type; referred as PPI task~\cite{airola2008all,tikk2010comprehensive,peng2017deep,hsieh2017identifying}. 
	

	
% It is also interesting to note that, when deploying an extraction model for processing text of million of articles to build models on biopathways~\cite{cohen2015darpa}, 
% 
% As done in previous works~\cite{airola2008all,tikk2010comprehensive,garg2016extracting,garg2018stochastic}, rather than using raw text, one can also obtain a syntactic or semantic parse of a given sentence as feature set.
	


==> rf_pseudo_code.tex <==
\begin{algorithm}[tp!]
\caption{
\csizenine
% 
KLSHRandomSubspaces
% 
% % Our 
% % Algorithm for 
% % Building Random Forest 
% Classification with 
% % from 
% Random Subsets of HashCodes Bits
% 
}
\csizenine
\begin{algorithmic}[1]
\REQUIRE Hashcodes of NLP structures $\bs{S}$ in training set, $\bs{C}$, and the corresponding class labels, $\bs{y}$;
% 
% Training data set, $\{ \bs{S}, \bs{y} \}$; reference set $\bs{S}^R$ of size $M$;
% 
% of natural language structures, $\bs{S} = \{ S_1, \cdots, S_N \}$ and their corresponding   labels $y_1, \cdots, y_N$;
% number of total hashcode bits, $H$; 
% 
number of bits for a random subspace, $\eta$; 
% size of reference set, $M$; 
% 
number of random subspaces, $R$.
% 
\\
% \STATE $\bs{r}^d \gets$ randomSubset($N$, $M$)
%
% % 
% \FOR{$i=1$ to $N$}
% % \STATE $\bs{c}_i \gets$ computeKLSHCode($S_i$, $\bs{S}(\bs{r}^d)$)
% \STATE $\bs{c}_i \gets$ computeKLSHCode($S_i$, $\bs{S}^{R}$)
% \ENDFOR
% % 
% 
% 
% \STATE $\bs{C} \gets$ computeKLSHCodes($\bs{S}$, $\bs{S}^{R}$)
% 
\STATE \COMMENT{Learning an ensemble of $R$ classifiers}
\FOR{$p = 1$ to $R$}
\label{alg:rnd_subspaces}
% 
% 
% \STATE $\bs{r}^c_j \gets$ randomSubset($H$, $\beta$)
% \label{alg:random_subset_bits}
% \COMMENT{a random subspace}
% \STATE ${DT}_j \gets$ learnDecisionTree($\{\bs{c}_1(\bs{r}^c_j), \cdots, \bs{c}_N(\bs{r}_j) \}$, $\bs{y}$)
% 
% 
\STATE $\bs{r}^c_p \gets$ randomSubset($H, \eta$)\COMMENT{sample $\eta$ elements randomly from from set $\{1, \cdots, H\}$}
% 
\STATE ${Clf}_p \gets$ trainClassifier($\bs{C}(:, \bs{r}^c_p), \bs{y}$)\COMMENT{train a classifier, using $\bs{C}(:, \bs{r}^c_p)$ as features}
% 
\ENDFOR
\RETURN $\{ {Clf}_p \}_{p=1}^R$, $\{\bs{r}_p^c\}_{p=1}^R$\COMMENT{the random subsets, $\{\bs{r}_p^c\}_{p=1}^R$, are used later to take subsets of $\bs{c}_*$ for inference}
\end{algorithmic}
\label{alg:our_algo}
% \vspace{-4mm}
\end{algorithm}


==> tab_extractions_ex.tex <==
\begin{table}
\centering
\csizenine
% \fontsize{7.8}{7.8}\selectfont
% \renewcommand{\arraystretch}{0.9}% Tighter
%	\renewcommand{\tabcolsep}{1.2pt}
%	\begin{tabular}{l}
% 
\begin{tabular}{p{7.5cm}}
% 
\toprule
Under normal \underline{signaling} conditions, \cat{\underline{Ras}} \underline{activation} helps mediate these events by
\underline{recruiting} the \underline{Raf} proteins to the plasma membrane, which induces the release
of \underline{14-3-3} from the N-terminal \underline{binding} site and facilitates \inte{\underline{phosphorylation}} of
the \pro{\underline{Raf kinase}} domain (19).\\
\midrule
\cat{\underline{Ras}} acts as a molecular switch that is \underline{activated} upon \underline{GTP} loading and
\underline{deactivated} upon \inte{\underline{hydrolysis}} of \pro{\underline{GTP}} to \underline{GDP}.\\
% 
 \midrule
 \pro{\underline{Ras}} proteins in their \cat{\underline{GTP}} state exist in \inte{\underline{complexes}} with effectors (\underline{Raf
 kinases}, \underline{RalGDS}, \underline{PI3K}, other \underline{Ras}-\underline{binding} proteins), as well as regulators
 (\underline{GAPs} and \underline{guanine nucleotide exchange factors} [\pro{\underline{GEFs}}]).
\\
\toprule
\end{tabular}
\vspace{-2.75mm}
\caption{
\csizeten
Some examples on extracting information on bio-molecular interactions from text sentences. In each text sentence, all tokens corresponding to a bio-entity~(proteins, molecules, chemicals, etc) or an interaction type are underlined. 
% 
While there can be multiple bio-molecular interactions mentioned in a sentence, we highlight one extraction in each sentence, that is 
% 
% A bio-molecular interaction is 
highlighted with color coding for its constituents: an interaction type~(in blue), and bio-entities either participating in the interaction~(in green), or catalyzing it~(in orange).
% 
}
\label{tab:ex_protein_pairs_extraction}
% \vspace{-0.5mm}
\end{table}
		

==> tab_notations.tex <==
% 
\begin{table}[tp!]
\centering
\csize
% \renewcommand{\arraystretch}{0.7}
\renewcommand{\tabcolsep}{2.0pt}
% 
\begin{tabular}{ll}
		\toprule
		Notation&Description\\
% 
\toprule
$S_i$&NLP structure, such as path, sequence, graph, etc\\
% \midrule
$\bs{S}$&NLP structures in training set, $\{S_1, \cdots, S_N\}$\\
% \midrule
$\bs{y}$&Class labels for $\bs{S}$ in training set, $\{ y_1, \cdots, y_N \}$\\
% \midrule
$\bs{S}^R$&Reference set of unlabeled NLP structures\\
% \midrule
$M$&Number of elements in $\bs{S}^R$\\
% \midrule
$\bs{c}_i$&Kernel-hashcode of NLP structure $S_i$\\
% \midrule
$\bs{k}_i$&Kernel similarity vector of $S_i$ w.r.t. $\bs{S}^R$\\
% \midrule
$\mhk$&Kernel-hashing model\\
% \midrule
$f_{\mhk}$&Kernel-hashing choice in $\mhk$~(RkNN, RMM, Kulis)\\
% \midrule
$h_l(.)$&$l_{th}$ kernel-hash function\\
% \midrule
$H$&Number of hash code bits~(functions)\\
% \midrule
$\gamma$&Number of samples to compute MI Lower Bound\\
$\beta$&Number of sampled candidates for greedy selection of $\bs{S}^R$\\
%
% \midrule
$\bs{S}^1_l$&Random subset of $\bs{S}^R$, to construct $h_l(.)$\\
% 
% \midrule
$\alpha$&Sampling parameter in $\mhk$; size of $\bs{r}^h_j$ is $2\alpha$\\
% \midrule
$R$&Number of random subspaces\\
% \midrule
$\eta$&Number of bits sampled for each random subspace\\
$\{M\}$&$\{1, \cdots, M\}$\\
$\cI(\bs{\cC}: \cY)$&Mutual information between hashcodes \& class labels\\
$\bar{\cI}(\bs{\cC}: \cY)$&Lower bound on $\cI(\bs{\cC}: \cY)$\\
% 
\toprule
\end{tabular}
\vspace{-3.25mm}
\caption{
\csizeten
% 
Some important notations.
}
\label{tab:notations}
\end{table}


==> tab_pubmed_bionlp_summary.tex <==
\begin{table}[tp!]
\centering
\csize
% \renewcommand{\arraystretch}{0.7}
% \renewcommand{\tabcolsep}{3.2pt}
% 
\begin{tabular}{llll}
		\toprule
		\textbf{Models}
       &\textbf{PubMed45}&\textbf{PubMed45-ERN}&\textbf{BioNLP}\\
%         &(Precision, Recall)\\
        \toprule
SVM~(Garg16)&$0.45$$\pm$$0.25$&$0.33$$\pm$$0.16$&$0.46$\\
        &(0.58, 0.43)&(0.33, 0.45)&(0.35, 0.67)\\
% \midrule
% SVM-PK&$0.557\pm0.201$\\
%         &(0.659, 0.513)\\
% 
% 
%         \midrule
%         kNN-PK&$0.44\pm0.18$\\
%         &(0.378, 0.646)\\
%         
%         \midrule
%         kNN
% %         -GK
%         &$0.45$$\pm$$0.16$&$0.26$$\pm$$0.15$&0.63\\
%         &(0.47, 0.51)&(0.26, 0.29)&(0.66, 0.59)\\
% % %         
% % 
% % 
% % 
% % k=1
% %         \toprule
% %         KLSH-kNN-PK~(M=100)&$0.350\pm0.173$\\
% %         &(0.308, 0.505)\\
% %       
% 
% 
\toprule
LSTM~(Rao17)&N.A.&N.A.&0.46\\
&&&(0.51, 0.44)\\
% 
% 
% 
        \midrule
% 
% KLSH-kNN~(M=100)\\
% \midrule
% 
% M=100
% 
% kNN based hashing
%         \toprule        
%         PK&$0.390\pm0.171$\\
%         &(0.349, 0.534)\\
% 
% 
% Kulis Hashing
%         \midrule
%         PK~(Kulis)&$0.406\pm0.188$\\
%         &(0.365, 0.540)\\
%         
% 
% SVM~(RMM) hashing
%         \midrule
% 
        KLSH-kNN
%         -PK
        &$0.46$$\pm$$0.21$&$0.23$$\pm$$0.13$&$0.60
%         \pm0.01
        $\\
        &(0.44, 0.53)&(0.23, 0.29)&(0.63, 0.57)\\
%         
% 
% 
% \midrule
% KLSH-kNN-NS*
% %         -PK
%         &$$$\pm$$$&$$$\pm$$$&$
% %         \pm0.01
%         $\\
%         &(, )&(, )&(, )\\
% %         
% 
% 
%         \toprule
% 
% kNN~(RMM) hashing
% 		\midrule
%         GK&$0.377\pm0.201$\\
%         &(0.371, 0.447)\\
%         
% 
% SVM~(RMM) hashing
% 
%         \midrule
%         KLSH-kNN-GK&$0.40\pm0.20$\\
%         &(0.40, 0.46)\\
% 
\toprule
% 
% \textbf{KLSH-RF*}&$\bs{0.55}$$\pm$$\bs{0.24}$&$\bs{0.43}$$\pm$$\bs{0.22}$&$\bs{0.63}
% % \pm
% % \bs{0.01}
% $\\
% &(\textbf{0.66, 0.50})&(\textbf{0.51, 0.47})&(\textbf{0.76, 0.54})\\
% % 
% 
% 
% % 
% % 
% % \midrule
% % optimized klsh config, and RF with MI LB
% \textbf{KLSH-RF}&$\bs{0.55}$$\pm$$\bs{0.24}$&$\bs{0.43}$$\pm$$\bs{0.22}$&$\bs{0.63}$\\
% % \pm
% % \bs{0.01}
% % \\
% &(\textbf{0.67, 0.49})&(\textbf{0.52, 0.46})&(\textbf{0.78, 0.52})\\
% % 
% % 
% % 
% % 
% % RMM
% % M=100
% % optimizing kernel, but fixed hash parameters
% % H=1000, R=250, alpha=2
% \midrule
% % PK
% \textbf{KLSH-RF$^+$~(PK)}&$\bs{0.57}$$\pm$$\bs{0.25}$&$\bs{0.42}$$\pm$$\bs{0.23}$&$\bs{0.63}$\\
% &(\textbf{0.63, 0.55})&(\textbf{0.46, 0.49})&(\textbf{0.78, 0.53})\\
% % 
% % 
% 
% % 
% % 
% % RMM
% % M=100
% % optimizing kernel, but fixed hash parameters
% % H=1000, R=100, alpha=2
% \midrule
% % GK
% \textbf{KLSH-RF$^+$~(GK)}&$\bs{0.55}$$\pm$$\bs{0.24}$&$\bs{0.45}$$\pm$$\bs{0.22}$&$\bs{0.60}$\\
% &(\textbf{0.65, 0.51})&(\textbf{0.51, 0.52})&(\textbf{0.81, 0.48})\\
% % 
% % 
% 
% RMM
% M=100
% optimizing kernel, but fixed hash parameters
% H=1000, R=100, alpha=2
% best of GK or PK
% \midrule
% 
% For BioNLP, Kulis and RkNN perform better for low value of alpha (2)
% so changing the values
% 
\textbf{KLSH-RF}&$\bs{0.57}$$\pm$$\bs{0.25}$&$\bs{0.45}$$\pm$$\bs{0.22}$
% kulis, 0.65~(not consistent for other datasets, keeping same hash that performs well across all datasets)
% &$\bs{0.65}$\\
&$\bs{0.63}$\\
&(\textbf{0.63, 0.55})&(\textbf{0.51, 0.52})
% &(\textbf{0.74, 0.58})\\
&(\textbf{0.78, 0.53})\\
% 
% 
\toprule
% 
\end{tabular}
\caption{Evaluation results for PubMed45  and BioNLP datasets. For each model, we report F1 score~(mean $\pm$ standard deviation) in the first row corresponding to it, and show mean-precision, mean-recall numbers as well, in brackets. For BioNLP, we don't show standard deviation since there is only one fixed test subset.}
\vspace{-3mm}
\label{tab:results_pubmed45_bionlp_all}
\end{table}



==> tab_results_aimed.tex <==
\begin{table}[tp!]
\centering
\tabsize
\subtable[
\tabsizesix
Other Models
]
{
\centering
\tabsizesix
\renewcommand{\arraystretch}{0.6}
\renewcommand{\tabcolsep}{1pt}
\begin{tabular}{ll}
		\toprule
		\textbf{Models}&\textbf{F1}\\
        &(P, R)\\
        \toprule
		SVM
%         -GK
%         ~\cite{garg2016extracting}
        ~[Garg2016]
        &0.39$\pm$0.05\\
        &(0.53, 0.33)\\
%         
% 
\midrule
kNN-PK&0.569$\pm$0.074\\
        &(0.499, 0.685)\\
% 
% 
\midrule
KLSH-kNN-PK&$\pm$\\
        &(, )\\
% 
% 
%         \toprule
%         Our KLSH-RF-PK\\
%         \midrule
%         M=500&$0.495\pm0.042$\\
%         &(0.539, 0.477)\\
%         \midrule
%         M=100&$0.522\pm0.058$\\
%         &(0.503, 0.566)\\
%         \midrule
%         M=30&$0.540\pm0.074$\\
%         &(0.493, 0.628)\\
% 
% 
        \toprule
\end{tabular}
}
\hspace{-3.25mm}
\subtable[
\tabsizesix
Our KLSH-RF with PK
]
{
\centering
\tabsizesix
\renewcommand{\arraystretch}{0.6}
\renewcommand{\tabcolsep}{1pt}
\begin{tabular}{ll}
		\toprule
		\textbf{Models}&\textbf{F1}\\
        &(P, R)\\
        \toprule
%         Our KLSH-RF-PK
% %         ~(ref chosen from all)
%         \\
% %         
% % 
% %         \midrule
%         M=500~(Kulis)&$\pm$\\
%         &(, )\\
%         
%         \midrule
        M=100~(RMM)&0.533$\pm$0.050\\
        &(0.519, 0.566)\\
%         
% 
%         \midrule
%         M=500&0.522$\pm$0.050\\
%         &(0.516, 0.549)\\
        \midrule
        M=100&0.545$\pm$0.070\\
        &(0.494, 0.635)\\
        \midrule
		M=30&\textbf{0.554}$\pm$0.082\\
        &(0.486, 0.671)\\
%         
% 
% 
        \toprule
\end{tabular}
}
\hspace{-3.25mm}
\subtable[
\tabsizesix
Our KLSH-RF~(Opt. MI LB)
]
{
\centering
\tabsizesix
\renewcommand{\arraystretch}{0.6}
\renewcommand{\tabcolsep}{1pt}
\begin{tabular}{ll}
		\toprule
		\textbf{Models}&\textbf{F1}\\
        &(P, R)\\
        \toprule
		\textbf{NS}-PK~(M=100)
%         ~(1e-4, chicago-trn)
        &\textbf{0.557}$\pm$0.072\\
        &(0.484, 0.685)\\
%         
% 
%         \midrule
% 		M=500~(RO)&0.532$\pm$0.045\\
%         &(0.518, 0.570)\\
% 
        \midrule
		\textbf{RO}-PK~(M=100)&0.538$\pm$0.072\\
        &(0.490, 0.626)\\
%         
        \midrule
		\textbf{RO}-PK~(M=30)&\textbf{0.561}$\pm$0.090\\
        &(0.483, 0.705)\\
% 
% 
        \toprule
\end{tabular}
}
\vspace{-4.5mm}
\caption{
Evaluation for AIMed dataset.
}
\label{tab:results_bionlp}
% \vspace{-2mm}
\end{table}


==> tab_results_bionlp.tex <==

% \begin{table*}[tp!]
% \centering
% \caption{
% Evaluation for BioNLP dataset.
% \todo{Show these results in many figures.}
% }
% \vspace{-4.75mm}
% % \small
% \scriptsize
% \subtable[
% \tabsize
% \textbf{Other Models}
% ]
% {
% \centering
% \tabsizemin
% \renewcommand{\arraystretch}{0.6}
% % \renewcommand{\arraystretch}{0.99}
% \renewcommand{\tabcolsep}{3.0pt}
% \begin{tabular}{ll}
% 		\toprule
% 		\textbf{Models}&\textbf{F1 Score}\\
%         &(Precision, Recall)\\
%         \toprule
%         SVM&$0.46$\\
%         &(0.35, 0.67)\\        
% 		\midrule        
%         LSTM~\cite{raobiomedical}&0.46\\
%         &(0.51, 0.44)\\
% %         
% \midrule
% kNN-PK&$0.63$\\
% &(0.66, 0.59)\\
% % 
% \midrule
% kNN-GK&$0.59$\\
% &(0.66, 0.54)\\
% % 
% % 
% % 
% % M=100
% %
% % kNN hashing
%         \midrule
%         KLSH-kNN-PK&$0.60\pm0.01$\\
%         &(0.63, 0.57)\\
% %         
% % Kulis hashing
% %         \midrule
% %         KLSH-kNN-PK~(Kulis)&$0.601\pm0.005$\\
% %         &(0.637, 0.569)\\
% %         
% % SVM (RMM) hashing
% %         \midrule
% %         KLSH-kNN-PK~(RMM)&$0.597\pm0.007$\\
% %         &(0.701, 0.519)\\
% %         
% % 
% % kNN hashing
% %         \midrule
% %         KLSH-kNN-GK&$0.552\pm0.011$\\
% %         &(0.594, 0.516)\\
% % 
% % Kulis hashing doesn't work as it leads to too many data points in same hash bucket
% % 
% % SVM (RMM) hashing
% \midrule
%         KLSH-kNN-GK&$0.56\pm0.01$\\
%         &(0.60, 0.52)\\
% 		\toprule
% \end{tabular}
% \label{tab:bionlp_others}
% }
% %         
% % 
% \subtable[
% \tabsize
% Our KLSH-RF with GK
% ]
% {
% \centering
% \tabsizemin
% \renewcommand{\arraystretch}{1.07}
% \renewcommand{\tabcolsep}{3.0pt}
% \begin{tabular}{ll}
% 		\toprule
% 		\textbf{Models}&\textbf{F1 Score}\\
%         &(Precision, Recall)\\
%         \toprule
% %         Our KLSH-RF-GK\\
% %         \midrule
%         M=500~(Kulis)&$0.47\pm0.04$\\
%         &(0.36, 0.69)\\
%         \midrule
%         M=500~(RMM)&$\bs{0.59}\pm0.00$\\
%         &(0.79, 0.48)\\
%         \midrule
%         M=500&$0.57\pm0.00$\\
%         &(0.75, 0.46)\\
%         \midrule
%         M=100&$0.58\pm0.02$\\
%         &(0.62, 0.54)\\
%         \midrule
%         M=30&$0.57\pm0.02$\\
%         &(0.55, 0.60)\\
% 		\toprule
% \end{tabular}
% \label{tab:bionlp_gk}
% }
% % 
% % 
% \subtable[
% \tabsize
% Our KLSH-RF with PK
% ]
% {
% \centering
% \tabsizemin
% \renewcommand{\arraystretch}{1.07}
% \renewcommand{\tabcolsep}{3.0pt}
% \begin{tabular}{ll}
% 		\toprule
% 		\textbf{Models}&\textbf{F1 Score}\\
%         &(Precision, Recall)\\
%         \toprule
% %         Our KLSH-RF-PK\\
% %         \midrule
%         M=500~(Kulis)&$0.62\pm0.00$\\
%         &(0.76, 0.52)\\
%         \midrule
%         M=500~(RMM)&$0.61\pm0.01$\\
%         &(0.80, 0.50)\\
%         \midrule
%         M=500&$\bs{0.63}\pm0.01$\\
%         &(0.76, 0.54)\\
%         \midrule
%         M=100&$0.62\pm0.01$\\
%         &(0.65, 0.60)\\
%         \midrule
%         M=30&$0.61\pm0.02$\\
%         &(0.61, 0.61)\\
% % 
% 		\toprule
% \end{tabular}
% \label{tab:bionlp_pk}
% }
% % 
% % 
% \subtable[
% \tabsize
% Our KLSH-RF Opt. with MI LB
% ]
% {
% \centering
% \tabsizemin
% \renewcommand{\arraystretch}{1.07}
% \renewcommand{\tabcolsep}{3.0pt}
% \begin{tabular}{ll}
% 		\toprule
% 		\textbf{Models}&\textbf{F1 Score}\\
%         &(Precision, Recall)\\
%         \toprule
%         \textbf{NS}-GK
% %         ~(3e-4)
%         ~(M=100)&$0.59\pm0.02$\\
%         &(0.63, 0.56)\\
%         \midrule
%         \textbf{NS}-PK
% %         ~(3e-4)
%         ~(M=100)&$0.63\pm0.01$\\
%         &(0.62, 0.64)\\
%         \midrule
% % 
% % greedy ss 300 rss 1000
% %         \midrule
%         \textbf{RO}-PK~(M=500)&$0.63$\\
%         &(0.76, 0.54)\\
%         \midrule
%         \textbf{RO}-PK~(M=100)&$0.63$\\
%         &(0.71, 0.58)\\
%         \midrule
%         \textbf{RO}-PK~(M=30)&$0.63$\\
%         &(0.70, 0.57)\\
% % %     
% % 
% % % old opt. as per AAAI-18 draft
% %         \midrule
% %         M=30~(RO)&$0.628\pm0.009$\\
% %         &(0.678, 0.585)\\
% % %         
% % 
% %         
% % 
% %         \toprule
% %         Our NS-KLSH-RF-PK\\
% %         \midrule
% % M=100&$\bs{0.625\pm0.012}$\\
% %         &(0.627, 0.625)\\
% 		\toprule
% \end{tabular}
% \label{tab:bionlp_opt_milb}
% }
% \label{tab:results_bionlp}
% \vspace{-8.5mm}
% \end{table*}
% % 

==> tab_results_pubmed_compressed.tex <==
% \begin{table*}[tp!]
% \centering
% \caption{
% Evaluation for PubMed45 dataset.
% }
% \vspace{-4.5mm}
% % \scriptsize
% % \small
% \subtable[
% \tabsize
% Other Models
% ]
% {
% \centering
% \tabsizemin
% \renewcommand{\arraystretch}{0.45}
% \renewcommand{\tabcolsep}{3.0pt}
% \begin{tabular}{ll}
% 		\toprule
% 		\textbf{Models}&\textbf{F1}\\
%         &(P., R.)\\
%         \toprule
% SVM~\cite{garg2016extracting}&0.45$\pm$0.25\\
%         &(0.58, 0.43)\\
% %         
% % \midrule
% % SVM-PK&$0.557\pm0.201$\\
% %         &(0.659, 0.513)\\
% % 
% % 
%         \midrule
%         kNN-PK&0.442$\pm$0.183\\
%         &(0.378, 0.646)\\
% %         
%         \midrule
%         kNN-GK&0.447$\pm$0.162\\
%         &(0.470, 0.513)\\
% %         
% % 
% % 
% % 
% % k=1
% %         \toprule
% %         KLSH-kNN-PK~(M=100)&$0.350\pm0.173$\\
% %         &(0.308, 0.505)\\
% %       
% % 
% % 
%         \midrule
% % 
% % KLSH-kNN~(M=100)\\
% % \midrule
% % 
% % M=100
% % 
% % kNN based hashing
% %         \toprule        
% %         PK&$0.390\pm0.171$\\
% %         &(0.349, 0.534)\\
% % 
% % 
% % Kulis Hashing
% %         \midrule
% %         PK~(Kulis)&$0.406\pm0.188$\\
% %         &(0.365, 0.540)\\
% %         
% % 
% % SVM~(RMM) hashing
% %         \midrule
% % 
%         KLSH-kNN-PK&0.458$\pm$0.211\\
%         &(0.441, 0.533)\\
% %         
% % 
% %         \toprule
% % 
% % kNN~(RMM) hashing
% % 		\midrule
% %         GK&$0.377\pm0.201$\\
% %         &(0.371, 0.447)\\
% %         
% % 
% % SVM~(RMM) hashing
%         \midrule
%         KLSH-kNN-GK&0.398$\pm$0.203\\
%         &(0.399, 0.456)\\
%         \toprule
% \end{tabular}
% \label{tab:pubmed_others}
% }        
% \hspace{-1.5mm}
% \subtable[
% \tabsize
% Our KLSH-RF with GK
% ]
% {
% \centering
% \tabsizemin
% \renewcommand{\arraystretch}{0.45}
% \renewcommand{\tabcolsep}{3.0pt}
% \begin{tabular}{lll}
% 		\toprule
% 		\textbf{Models}&GK&PK\\
%         \toprule
% %         Our KLSH-RF-GK&\\
% %         \midrule
%         M=500~(Kulis)&$0.446\pm0.187$&$0.485\pm0.137$\\
%         &(0.353, 0.717)&(0.561, 0.489)\\
%         \midrule
%         M=500~(RMM)&$\bs{0.548}\pm0.240$&$\bs{0.518}\pm0.212$\\
%         &(0.656, 0.499)&(0.614, 0.476)\\
%         \midrule
%         M=500&$\bs{0.540}\pm0.236$&$\bs{0.486}\pm0.159$\\
%         &(0.624, 0.505)&(0.590, 0.458)\\
%         \midrule
%         M=100&$0.514\pm0.216$&$0.475\pm0.154$\\
%         &(0.517, 0.566)&(0.499, 0.522)\\
%         \midrule
%         M=30&$\bs{0.508}\pm0.220$&$0.473\pm0.164$\\
%         &(0.478, 0.615)&(0.458, 0.580)\\
% %         
% %         \midrule
% %         M=30~(RO)&$0.512\pm0.217$\\
% %         &(0.500, 0.592)\\
% % 
% % 
% % 
% % % subsample size 10 
% %         \toprule
% %         Our KLSH-RF-PK~(RMM)&\\
% %         \midrule
% %         M=500&$0.525\pm0.215$\\
% %         &(0.623, 0.483)\\
% %         \midrule
% %         M=100&$0.519\pm0.221$\\
% %         &(0.595, 0.493)\\
% % 
% % 
% % 
%         \toprule
% \end{tabular}
% \label{tab:pubmed_our_gk}
% }
% % \hspace{-1.5mm}
% % \subtable[
% % \tabsize
% % Our KLSH-RF with PK
% % ]
% % {
% % \centering
% % \tabsizemin
% % \renewcommand{\arraystretch}{0.45}
% % \renewcommand{\tabcolsep}{3.0pt}
% % \begin{tabular}{ll}
% % 		\toprule
% % 		\textbf{Models}&\textbf{F1 Score}\\
% %         &(Precision, Recall)\\
% %         \toprule
% % %         Our KLSH-RF-PK&\\
% % %         
% % %         \midrule
% % %         M=500~(RMM, RO)&$0.524\pm0.210$\\
% % %         &(0.617, 0.484)\\
% % % 
% % %         \midrule
% %         M=500~(Kulis)&$0.485\pm0.137$\\
% %         &(0.561, 0.489)\\
% %         \midrule
% %         M=500~(RMM)&$\bs{0.518}\pm0.212$\\
% %         &(0.614, 0.476)\\
% %         \midrule
% %         M=500&$\bs{0.486}\pm0.159$\\
% %         &(0.590, 0.458)\\
% %         \midrule
% %         M=100&$0.475\pm0.154$\\
% %         &(0.499, 0.522)\\
% %         \midrule
% %         M=30&$0.473\pm0.164$\\
% %         &(0.458, 0.580)\\
% % %         
% % % trained on PubMed using the old algo
% % %         \midrule
% % %         M=30~(RO)&$0.480\pm0.172$\\
% % %         &(0.486, 0.543)\\
% % %         
% % % 
% % % trained on PubMed ss 300 rss 1000
% % % 
% % % 
% % % 
% % % 
% % %         \midrule
% % %         trained on BioNLP-chicago
% % % ss 300 rss 1000
% % %         M=30~(RO)&$0.491\pm0.184$\\
% % %         &(0.478, 0.588)\\
% % % 
% % % 
% % %         \toprule
% % %         Our KLSH-RF-PK&\\
% % %         \midrule
% % %         M=500&$0.501\pm0.183$\\
% % %         &(0.554, 0.509)\\
% % %         \midrule
% % %         M=100&$0.483\pm0.204$\\
% % %         &(0.449, 0.599)\\
% % %         \midrule
% % %         M=30&$0.433\pm0.182$\\
% % %         &(0.346, 0.716)\\
% % %         \midrule
% % %         M=30~(RO)&$0.454\pm0.188$\\
% % %         &(0.376, 0.674)\\
% % %         \toprule
% % %         Our KLSH-RF-Word2Vec-RO&\\
% % %         \toprule
% % %         Our KLSH-RF-RO&\\
% % %         \midrule
% % %         M=30&$$\\
% % 		\toprule
% % \end{tabular}
% % \label{tab:pubmed_our_pk}
% % }
% \hspace{-1.5mm}
% \subtable[
% \tabsize
% Our KLSH-RF Opt. with MI LB
% ]
% {
% \centering
% \tabsizemin
% \renewcommand{\arraystretch}{0.45}
% \renewcommand{\tabcolsep}{3.0pt}
% \begin{tabular}{ll}
% 		\toprule
% 		\textbf{Models}&\textbf{F1}\\
%         &(P., R.)\\
%         \toprule
%         \textbf{NS}-GK~(M=100)
% %         -ChicagoBioNLP
%         &$\bs{0.526}$$\pm$0.222\\
%         &(0.527, 0.584)\\
% % 
%         \midrule
%         \textbf{NS}-PK~(M=100)
% %         -ChicagoBioNLP
%         &$\bs{0.493}\pm0.173$\\
%         &(0.505, 0.555)\\
% % 
% %         \toprule
% %         Our NS-KLSH-RF-PK\\
% %         \midrule
% % M=100&$\bs{0.493\pm0.173}$\\
% %         &(0.505, 0.555)\\
% % 
% % 
% % 
% \midrule
% \textbf{RO}-PK~(M=500)&$\bs{0.505}\pm0.218$\\
%         &(0.624, 0.446)\\
% % 
% \midrule
% \textbf{RO}-PK~(M=100)&$\bs{0.497}\pm0.157$\\
%         &(0.549, 0.511)\\
% % 
% % 
% \midrule
% \textbf{RO}-PK~(M=30)&$0.477\pm0.133$\\
%         &(0.486, 0.540)\\
% % 
% 		\toprule
% \end{tabular}
% \label{tab:pubmed_our_opt_milb}
% }
% \label{tab:results_pubmed45}
% \vspace{-8.5mm}
% \end{table*}

